Learning to Use Local Cuts

An essential component in modern solvers for mixed-integer (linear) programs (MIPs) is the separation of additional inequalities (cutting planes) to tighten the linear programming relaxation. Various algorithmic decisions are necessary when integrating cutting plane methods into a branch-and-bound (B&B) solver as there is always the trade-off between the efficiency of the cuts and their costs, given that they tend to slow down the solution time of the relaxation. One of the most crucial questions is: Should cuts only be generated globally at the root or also locally at nodes of the tree? We address this question by a machine learning approach for which we train a regression forest to predict the speed-up (or slow-down) provided by using local cuts. We demonstrate with an open implementation that this helps to improve the performance of the FICO Xpress MIP solver on a public test set of general MIP instances. We further report on the impact of a practical implementation inside Xpress on a large, diverse set of real-world industry MIPs.

==> Classification_Tab.tex <==
\begin{tabular}{|c|c|c|cc|cc|}
\hline
& \textbf{Ver} & \M & \always & \texttt{Oracle} & \textbf{Imp} ($\%$) & \textbf{Gap} ($\%$) \\
\hline
\hline
& Reg & \textbf{427.91} & \multirow{2}{*}{467.92} & \multirow{2}{*}{414.75} & -8.55 & -75.25 \\  
\multirow{-2}{*}{\emph{Train}} 
& Class & 435.00 &  &  & -7.04 & -61.91\\
\hline
\hline
& Reg & \textbf{420.09} & & & -3.34 & -29.10 \\  
\multirow{-2}{*}{\emph{Test}}  & Class & 432.54 & \multirow{-2}{*}{434.61}  & \multirow{-2}{*}{384.72} & -1.47 & -12.79 \\
\hline
\end{tabular}

==> Features_Tab.tex <==
\begin{tabular}{|p{0.15cm}|p{3.3cm}|p{4.77cm}|p{3.5cm}|p{4.77cm}|}  
\hline
& \textbf{Feature} & \textbf{Definition} & \textbf{Feature} & \textbf{Definition} \\
\hline
\hline
& \multicolumn{4}{c|}{\emph{$\sim$ Matrix $\sim$}} \\
\hhline{~ *{4}{-}}
& \texttt{Rows} & $\ln(m)$ & \texttt{NonZeros} & ratio of non-zeros, over $m\times n$ \\
& \texttt{Columns} & $\ln(n)$ & \texttt{Symmetries} & $1$ if any simmetry, $0$ otherwise \\
\hhline{~ *{4}{-}}
& \multicolumn{4}{c|}{\emph{$\sim$ Variables $\sim$}} \\
\hhline{~ *{4}{-}}
& \texttt{Binaries} & ratio of binary variables, over $n$ & \texttt{Integers} & ratio of integer variables, over $n$ \\
\hhline{~ *{4}{-}}
& \multicolumn{4}{c|}{\emph{$\sim$ Constraints $\sim$}} \\
\hhline{~ *{4}{-}}
& \texttt{LessThan} & \multirow{8}{4cm}{Ratio of constraints per constraint type, over $m$} & \texttt{Knapsack} & \multirow{8}{4cm}{Ratio of constraints per constraint type, over $m$} \\
& \texttt{GreaterThan} & & \texttt{KnapsackInteger} & \\
& \texttt{Equality} & & \texttt{BinaryPacking} &  \\
& \texttt{SetPartitioning} & & \texttt{VariableLowerBound} & \\
& \texttt{SetPacking} & & \texttt{VariableUpperBound} &  \\
& \texttt{SetCovering} & & \texttt{MixedBinary} & \\
& \texttt{Cardinality} & & \texttt{MixedInteger} & \\
& \texttt{KnapsackEquality} & & \texttt{Continuous} & \\
\hhline{~ *{4}{-}}
& \multicolumn{4}{c|}{\emph{$\sim$ Numerics $\sim$}} \\
\hhline{~ *{4}{-}}
& \texttt{Coefficient\_Oom} & $\ln(\max A^{\prime} / \min A^{\prime})$ & \texttt{Objective\_Oom} & $\ln(\max c^{\prime} / \min c^{\prime})$ \\
\multirow{-16}{*}{\rotatebox[origin=c]{90}{\textnormal{\emph{\textbf{Static}}}}} & \texttt{RightHandSide\_Oom} & $\ln(\max b^{\prime} / \min b^{\prime})$ & & \\
\hline
& \multicolumn{4}{c|}{\emph{$\sim$ Presolving $\sim$}} \\
\hhline{~ *{4}{-}}
& \texttt{PresolRows} & $\ln(\tilde{m})$ & \texttt{PresolIntegers} & ratio of presolved integer variables, over $n$ \\
& \texttt{PresolColumns} & $\ln(\tilde{n})$ & &  \\
\hhline{~ *{4}{-}}
& \multicolumn{4}{c|}{\emph{$\sim$ GlobalCuts $\sim$}} \\
\hhline{~ *{4}{-}}
& \texttt{DualInitial\_Gap} & $\lvert\dualbound - \initbound\rvert/\max(\lvert \dualbound \rvert, \lvert \initbound \rvert, \lvert \dualbound-\initbound\rvert)$ & \texttt{PrimalInitial\_Gap} & $\lvert\primalbound - \initbound\rvert/\max(\lvert\primalbound\rvert, \lvert\initbound\rvert, \lvert\primalbound-\initbound\rvert)$ \\
\multirow{-6}{*}{\rotatebox[origin=c]{90}{\emph{\textbf{Dynamic}}}} &  \texttt{PrimalDual\_Gap} & $\lvert\primalbound - \dualbound\rvert/\max(\lvert\primalbound\rvert,\lvert \dualbound\rvert, \lvert\primalbound-\dualbound\rvert)$ & \texttt{Gap\_Closed} & $1 - \frac{\texttt{PrimalDual\_Gap}}{\texttt{DualInitial\_Gap}}$ \\
\hline
\end{tabular}


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


